Travel the Same Path: A Novel TSP Solving Strategy

In this paper, we provide a novel strategy for solving Traveling Salesman Problem, which is a famous combinatorial optimization problem studied intensely in the TCS community. In particular, we consider the imitation learning framework, which helps a deterministic algorithm making good choices whenever it needs to, resulting in a speed up while maintaining the exactness of the solution without suffering from the unpredictability and a potential large deviation. Furthermore, we demonstrate a strong generalization ability of a graph neural network trained under the imitation learning framework. Specifically, the model is capable of solving a large instance of TSP faster than the baseline while has only seen small TSP instances when training.

==> dataset_generation.tex <==
Also, we have implement the code template which split the data into training set, validation and also testing set and wrapped them up.
Here is the output.
\begin{lstlisting}[style=DOS]
seed 0
1000 train instances for 1000 samples
200 validation instances for 200 samples
0 test instances for 200 samples
[w Thread-2] episode 0, seed 3789440165, processing instance 'data/instances/setcover/train_500r_1000c_0.05d/instance_154.lp'...
[w Thread-3] episode 1, seed 3998999672, processing instance 'data/instances/setcover/train_500r_1000c_0.05d/instance_651.lp'...
[w Thread-4] episode 2, seed 3665041058, processing instance 'data/instances/setcover/train_500r_1000c_0.05d/instance_364.lp'...
[w Thread-5] episode 3, seed 2122579412, processing instance 'data/instances/setcover/train_500r_1000c_0.05d/instance_829.lp'...
[w Thread-4] episode 2 done, 3 samples
[w Thread-4] episode 4, seed 92199959, processing instance 'data/instances/setcover/train_500r_1000c_0.05d/instance_706.lp'...
[m MainThread] 1 / 1000 samples written, ep 0 (4 in buffer).
[m MainThread] 2 / 1000 samples written, ep 0 (4 in buffer).
[m MainThread] 3 / 1000 samples written, ep 0 (4 in buffer).
...
[m MainThread] 111 / 1000 samples written, ep 0 (226 in buffer).
[m MainThread] 112 / 1000 samples written, ep 0 (231 in buffer).
[m MainThread] 113 / 1000 samples written, ep 0 (233 in buffer).
[w Thread-2] episode 0 done, 113 samples
[w Thread-2] episode 5, seed 3084161443, processing instance 'data/instances/setcover/train_500r_1000c_0.05d/instance_492.lp'...
...
[m MainThread] 999 / 1000 samples written, ep 1 (2899 in buffer).
[m MainThread] 1000 / 1000 samples written, ep 1 (2901 in buffer).
[w Thread-7] episode 0, seed 4086331612, processing instance 'data/instances/setcover/valid_500r_1000c_0.05d/instance_116.lp'...
[w Thread-8] episode 1, seed 4177056010, processing instance 'data/instances/setcover/valid_500r_1000c_0.05d/instance_34.lp'...
[w Thread-9] episode 2, seed 1004525138, processing instance 'data/instances/setcover/valid_500r_1000c_0.05d/instance_36.lp'...
[w Thread-10] episode 3, seed 2483450156, processing instance 'data/instances/setcover/valid_500r_1000c_0.05d/instance_14.lp'...
[w Thread-4] episode 14 done, 1078 samples
[m MainThread] 1 / 200 samples written, ep 0 (5 in buffer).
[m MainThread] 2 / 200 samples written, ep 0 (8 in buffer).
[m MainThread] 3 / 200 samples written, ep 0 (12 in buffer).
...
\end{lstlisting}

==> instance_generation.tex <==
After utilizing the Ecole library, we have tried to generate some sample problem instances for \texttt{setcover}. Here is the result.
\begin{lstlisting}[style=DOS]
1000 instances in data/instances/setcover/train_500r_1000c_0.05d
200 instances in data/instances/setcover/valid_500r_1000c_0.05d
10 instances in data/instances/setcover/transfer_50r_1000c_0.05d
10 instances in data/instances/setcover/transfer_100r_1000c_0.05d
10 instances in data/instances/setcover/transfer_200r_1000c_0.05d
200 instances in data/instances/setcover/test_50r_100c_0.05d
  generating file data/instances/setcover/train_500r_1000c_0.05d/instance_1.lp ...
  generating file data/instances/setcover/train_500r_1000c_0.05d/instance_2.lp ...
  generating file data/instances/setcover/train_500r_1000c_0.05d/instance_3.lp ...
  ...
  generating file data/instances/setcover/train_500r_1000c_0.05d/instance_999.lp ...
  generating file data/instances/setcover/train_500r_1000c_0.05d/instance_1000.lp ...
  generating file data/instances/setcover/valid_500r_1000c_0.05d/instance_1.lp ...
  generating file data/instances/setcover/valid_500r_1000c_0.05d/instance_2.lp ...
  generating file data/instances/setcover/valid_500r_1000c_0.05d/instance_3.lp ...
  ...
  generating file data/instances/setcover/valid_500r_1000c_0.05d/instance_199.lp ...
  generating file data/instances/setcover/valid_500r_1000c_0.05d/instance_200.lp ...
  generating file data/instances/setcover/transfer_50r_1000c_0.05d/instance_1.lp ...
  generating file data/instances/setcover/transfer_50r_1000c_0.05d/instance_2.lp ...
  generating file data/instances/setcover/transfer_50r_1000c_0.05d/instance_3.lp ...
  ...
  generating file data/instances/setcover/transfer_50r_1000c_0.05d/instance_9.lp ...
  generating file data/instances/setcover/transfer_50r_1000c_0.05d/instance_10.lp ...
  generating file data/instances/setcover/transfer_100r_1000c_0.05d/instance_1.lp ...
  generating file data/instances/setcover/transfer_100r_1000c_0.05d/instance_2.lp ...
  generating file data/instances/setcover/transfer_100r_1000c_0.05d/instance_3.lp ...
  ...
  generating file data/instances/setcover/transfer_100r_1000c_0.05d/instance_9.lp ...
  generating file data/instances/setcover/transfer_100r_1000c_0.05d/instance_10.lp ...
  generating file data/instances/setcover/transfer_200r_1000c_0.05d/instance_1.lp ...
  generating file data/instances/setcover/transfer_200r_1000c_0.05d/instance_2.lp ...
  generating file data/instances/setcover/transfer_200r_1000c_0.05d/instance_3.lp ...
  ...
  generating file data/instances/setcover/transfer_200r_1000c_0.05d/instance_9.lp ...
  generating file data/instances/setcover/transfer_200r_1000c_0.05d/instance_10.lp ...
  generating file data/instances/setcover/test_50r_100c_0.05d/instance_1.lp ...
  generating file data/instances/setcover/test_50r_100c_0.05d/instance_2.lp ...
  generating file data/instances/setcover/test_50r_100c_0.05d/instance_3.lp ...
  ...
  generating file data/instances/setcover/test_50r_100c_0.05d/instance_199.lp ...
  generating file data/instances/setcover/test_50r_100c_0.05d/instance_200.lp ...
done.
\end{lstlisting}
